Neural Operators Can Play Dynamic Stackelberg Games

Dynamic Stackelberg games are a broad class of two-player games in which the leader acts first, and the follower chooses a response strategy to the leader's strategy. Unfortunately, only stylized Stackelberg games are explicitly solvable since the follower's best-response operator (as a function of the control of the leader) is typically analytically intractable. This paper addresses this issue by showing that the \textit{follower's best-response operator} can be approximately implemented by an \textit{attention-based neural operator}, uniformly on compact subsets of adapted open-loop controls for the leader. We further show that the value of the Stackelberg game where the follower uses the approximate best-response operator approximates the value of the original Stackelberg game. Our main result is obtained using our universal approximation theorem for attention-based neural operators between spaces of square-integrable adapted stochastic processes, as well as stability results for a general class of Stackelberg games.

==> Cover_Letter.tex <==
 %!TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Neural Operators Can Play Dynamic Stackelberg Games}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies the ability of neural operators (NOs) to approximate the best response map to dynamic Stackelberg games in continuous time with general dynamics.  Our results are all quantitative, and we identify structures on the sets of admissible actions of the leader, which imply feasible approximation rates for the NO.

These results are significant since they are the first class of results which show that one can learn how to play (best response map) extremely complicated Stackelberg games for which classical analytical methods are unavailalbe.  Our results also show that Neural Operators can be used to solve problems in other areas than PDEs, where PINNs-type NOs are most explored.  Further, our paper introduces NOs classes that map between spaces of adapted processes ideal for optimal control.

Our quantitative approximation rates for NOs allow us to identify sets of admissible controls for the leader on which NOs can efficiently approximate the best response map.  
Interestingly, this class consists of appropriate open-loop perturbations of closed-loop solutions to a linear-quadratic proxy of our general Stackelberg game.  This later pioneering connection between operator learning and game theory shows that we can learn about ``what simple actions are'' from our approximation-theoretic insights.
% 
On the technical side, we also derive new stability/regularity results for the best response map of rather general Stackelberg games.

This paper is not an extension of an earlier conference paper. 

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{Sayan Mukherjee
, Max Planck Institute (sayan.mukherjee@mis.mpg.de)}
    \item \red{Daniel Roy
, University of Toronto (daniel.roy@utoronto.ca
)}
    \item \red{Ambuj Tewari
, University of Michigan (tewaria@umich.edu)}
    \item \red{Mehryar Mohri, New York University (mohri@cs.nyu.edu)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Our submission has the following keywords: \red{keyword}, \red{keyword}, \red{keyword}, \red{keyword}, \red{keyword}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Guillermo Alonso Alvarez (University of Michigan)}\\
\red{Ibrahim Ekren (University of Michigan)}\\
\red{Anastasis Kratsios (Institution)}\\
\red{Xuwei Yang (Institution)}

% \title{Cover letter}
% \author{
% }
% \date{} % delete this line to display the current date

% %%% BEGIN DOCUMENT
% \begin{document}

% \maketitle

% \begin{enumerate}
% \item This paper is not an extension of an earlier conference paper. 
% \item All co-authors are aware of the current submission and consent to its review by JMLR.
% \item No possible conflicts of interest. 
% \item Action editor: .....
% \item Reviewer: ....
% \item Keywords: 
% \end{enumerate}



\end{document}







































